Atomic Layer Epitaxy of Kagome Magnet Fe${_3}$Sn${_2}$ and Sn-modulated Heterostructures

Magnetic materials with kagome crystal structure exhibit rich physics such as frustrated magnetism, skyrmion formation, topological flat bands, and Dirac/Weyl points. Until recently, most studies on kagome magnets have been performed on bulk crystals or polycrystalline films. Here we report the atomic layer molecular beam epitaxy synthesis of high-quality thin films of topological kagome magnet Fe${_3}$Sn${_2}$. Structural and magnetic characterization of Fe${_3}$Sn${_2}$ on epitaxial Pt(111) identifies highly ordered films with c-plane orientation and an in-plane magnetic easy axis. Studies of the local magnetic structure by anomalous Nernst effect imaging reveals in-plane oriented micrometer size domains. Superlattice structures consisting of Fe${_3}$Sn${_2}$ and Fe${_3}$Sn are also synthesized by atomic layer molecular beam epitaxy, demonstrating the ability to modulate the sample structure at the atomic level. The realization of high-quality films by atomic layer molecular beam epitaxy opens the door to explore the rich physics of this system and investigate novel spintronic phenomena by interfacing Fe${_3}$Sn${_2}$ with other materials.

==> figures/gnuplot_XRD_Fe3Sn2_growth_temps_series <==
#! /usr/bin/gnuplot -persist
scale = 1
set terminal pdfcairo enhanced font "Helvetica Bold, 38" size 10*scale,8*scale

set encoding default
set nokey
set xlabel "2θ (deg)"
set ylabel "Intensity (cps)"
set logscale y 10
set xrange [9:98]
set xtics 10 scale 1.2
set mxtics 5
set format x "%2.0f"
set format y "10^{%L}" 
y0 = -0.0
set yrange [1:1E+45]
set ytics 1E+5 scale 1.2
#set mytics 1E+4
set border lw 4*scale
set key top right
#set autoscale 

set ylabel offset -1,0
set xlabel offset 0,0

set style line 1 lc "black" lw 8*scale pt 6 ps 0.0
set style line 2 lc "red" lw 6*scale pt 7 ps 0.0
set style line 3 lc "blue" lw 2*scale pt 7 ps 0.0
set style line 4 lc "green" lw 8*scale pt 6 ps 0.00
set style line 5 lc "orange" lw 4*scale pt 6 ps 0.0
set style line 6 lc "magenta" lw 4*scale pt 6 ps 0.0

#-----------------------------------------------------------------------------------------

sample_id_RT1 = "Fe3Sn2_20210216"
data_file_RT1 = sample_id_RT1."_XRD_scan.txt"

sample_id_RT2 = "Fe3Sn2_20210413"
data_file_RT2 = sample_id_RT2."_XRD_scan.txt"

sample_id_RT3 = "Fe3Sn2_20210726"
data_file_RT3 = sample_id_RT3."_XRD_scan.txt"

sample_id_70C = "Fe3Sn2_20210719"
data_file_70C = sample_id_70C."_XRD_scan.txt"

sample_id_100C = "Fe3Sn2_20210721"
data_file_100C = sample_id_100C."_XRD_scan.txt"

sample_id_150C = "Fe3Sn2_20210718"
data_file_150C = sample_id_150C."_XRD_scan.txt"

set output "Fe3Sn2_XRD_growth_temps_series_with_peak_labels.pdf"

lambda = 1.54056 # in Angstroms

lattice_c = 12.991
d = lattice_c/sqrt(0**2+0**2+6**2)
m_sub = 1
x_sub = 2*asin(m_sub*lambda/2/d)*180/3.14159

d = lattice_c/sqrt(0**2+0**2+12**2)
x_sub_00012 = 2*asin(m_sub*lambda/2/d)*180/3.14159

x_peak = 41.2
m_peak = 2
d = m_peak/2.0*lambda/sin(x_peak/2*3.14159/180)
d_ref = 4.31 # literature
x_label = 37.5

lattice_c = 19.789
d = lattice_c/sqrt(0**2+0**2+9**2)
m_sub = 1
x_0009 = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 19.789
d = lattice_c/sqrt(0**2+0**2+3**2)
m_sub = 1
x_0003 = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 19.789
d = lattice_c/sqrt(0**2+0**2+6**2)
m_sub = 1
x_0006 = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 19.789
d = lattice_c/sqrt(0**2+0**2+18**2)
m_sub = 1
x_00018 = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 3.924
d = lattice_c/sqrt(1**2+1**2+1**2)
m_sub = 1
x_111 = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 3.924
d = lattice_c/sqrt(2**2+2**2+2**2)
m_sub = 1
x_222 = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 4.362
d = lattice_c/sqrt(0**2+0**2+2**2)
m_sub = 1
x_0002_Fe3Sn = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 4.362
d = lattice_c/sqrt(0**2+0**2+4**2)
m_sub = 1
x_0004_Fe3Sn = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 4.440
d = lattice_c/sqrt(0**2+0**2+2**2)
m_sub = 1
x_0002_FeSn = 2*asin(m_sub*lambda/2/d)*180/3.14159

lattice_c = 4.440
d = lattice_c/sqrt(0**2+0**2+4**2)
m_sub = 1
x_0004_FeSn = 2*asin(m_sub*lambda/2/d)*180/3.14159

#set label sprintf("Al_2O_3(0006), %1.2f",lattice_c) at 39.8,1E+2 rotate by 90

set label "Al_2O_3(0006)" at x_sub,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Al_2O_3(0012)" at x_sub_00012,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Fe_3Sn2 (0009)" at x_0009,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Fe_3Sn2 (0003)" at x_0003,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Fe_3Sn2 (0006)" at x_0006,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Fe_3Sn2 (00018)" at x_00018,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Pt (111)" at x_111,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Pt (222)" at x_222,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Fe3Sn (0002)" at x_0002_Fe3Sn,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "FeSn (0002)" at x_0002_FeSn,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "Fe3Sn (0004)" at x_0004_Fe3Sn,1E+31 rotate by 90 font "Helvetica Bold, 20"
set label "FeSn (0004)" at x_0004_FeSn,1E+31 rotate by 90 font "Helvetica Bold, 20"

#set label sprintf ("2θ_{sub} = %2.2f",x_sub) at x_label,1E+3
#set label sprintf ("2θ_{Fe_3Sn} = %2.2f",x_peak) at x_label,3E+2
#set label sprintf ("d_{Fe_3Sn} = %2.2f Å",d) at x_label,1E+4
#set label sprintf ("d_{Fe_3Sn}^{ref} = %2.2f Å",d_ref) at x_label,3E+3

x_label = 13

set label "RT1" at x_label,1E+2 font "Helvetica Bold, 30"
set label "RT2" at x_label,1E+7 font "Helvetica Bold, 30"
set label "RT3" at x_label,1E+12 font "Helvetica Bold, 30"
set label "70 °C" at x_label,1E+17 font "Helvetica Bold, 30"
set label "100 °C" at x_label,1E+22 font "Helvetica Bold, 30"
set label "150 °C" at x_label,1E+27 font "Helvetica Bold, 30"

#set arrow from x_peak,1E+1 to x_peak,1E+2 ls 1 dt 1 lw 6 nohead 

plot data_file_RT1 using ($1*2+x_sub):(($2+1)*1E+0) w lines ls 3 notitle "RT1",\
data_file_RT2 using ($1*2/3600+x_sub):(($2+1)*1E+5) w lines ls 3 notitle "RT2",\
data_file_RT3 using ($1*2+x_sub):(($2+1)*1E+10) w lines ls 3 notitle "RT3",\
data_file_70C using ($1*2+x_sub):(($2+1)*1E+15) w lines ls 3 notitle "70 °C",\
data_file_100C using ($1*2+x_sub):(($2+1)*1E+20)w lines ls 3 notitle "100 °C",\
data_file_150C using ($1*2+x_sub):(($2+1)*1E+25) w lines ls 3 notitle "150 °C"


#------------------------------------------------------------------------------------------

set output "Fe3Sn2_XRD_growth_temps_series_with_peak_labels.png"

scale = 150

set terminal pngcairo enhanced font "Helvetica Bold, 38" size 10*scale,8*scale

plot data_file_RT1 using ($1*2+x_sub):(($2+1)*1E+0) w lines ls 3 notitle "RT1",\
data_file_RT2 using ($1*2/3600+x_sub):(($2+1)*1E+5) w lines ls 3 notitle "RT2",\
data_file_RT3 using ($1*2+x_sub):(($2+1)*1E+10) w lines ls 3 notitle "RT3",\
data_file_70C using ($1*2+x_sub):(($2+1)*1E+15) w lines ls 3 notitle "70 °C",\
data_file_100C using ($1*2+x_sub):(($2+1)*1E+20)w lines ls 3 notitle "100 °C",\
data_file_150C using ($1*2+x_sub):(($2+1)*1E+25) w lines ls 3 notitle "150 °C"

